An approximate likelihood for nuclear recoil searches with XENON1T data

The XENON collaboration has published stringent limits on specific dark matter -nucleon recoil spectra from dark matter recoiling on the liquid xenon detector target. In this paper, we present an approximate likelihood for the XENON1T 1 tonne-year nuclear recoil search applicable to any nuclear recoil spectrum. Alongside this paper, we publish data and code to compute upper limits using the method we present. The approximate likelihood is constructed in bins of reconstructed energy, profiled along the signal expectation in each bin. This approach can be used to compute an approximate likelihood and therefore most statistical results for any nuclear recoil spectrum. Computing approximate results with this method is approximately three orders of magnitude faster than the likelihood used in the original publications of XENON1T, where limits were set for specific families of recoil spectra. Using this same method, we include toy Monte Carlo simulation-derived binwise likelihoods for the upcoming XENONnT experiment that can similarly be used to assess the sensitivity to arbitrary nuclear recoil signatures in its eventual 20 tonne-year exposure.

==> xenon_authorlist_Dec21v3.tex <==
% Autogenerated on 08 Mar, 2022 at 14:36:03
% Generated with make-authorlist.py

% NOTE: there is a nasty bug in the PTEP style file! You need to replace the 
% newlogo.eps file with an essentially empty newlogo.png. If you don't the
% formatting of the authorlist becomes crooked. 
%
% -> SNIP
%\documentclass{ptephy_v1}
%\documentclass[sn-mathphys, iicol]{sn-jnl}% Math and Physical Sciences Reference Style
%\usepackage{currfile} % To be able to list current file name in title
%% <- SNIP
%
%
%\begin{document}
%
%% CHANGE TO TITLE
%\title{XENON Authors \currfilename}
\author[1]{E.~Aprile}
\author[2]{K.~Abe}
\author[3]{F.~Agostini}
\author[4]{{S.~Ahmed~Maouloud}}
\author[5]{{M.~Alfonsi}}
\author[6]{{L. Althueser}}
\author[4]{B. Andrieu}
\author[7]{E. Angelino}
\author[8]{J. R.~Angevaare}
\author[9]{V. C.~Antochi}
\author[10]{D. Ant\'on Martin}
\author[11]{F. Arneodo}
\author[12]{L. Baudis}
\author[13]{A.L. Baxter}
\author[3]{L. Bellagamba}
\author[14]{R. Biondi}
\author[12]{A. Bismark}
\author[15]{A. Brown}
\author[8]{S. Bruenner}
\author[11,16]{G. Bruno}
\author[17]{R. Budnik}
\author[12]{C. Capelli}
\author[18]{J. M. R. Cardoso}
\author[19]{D. Cichon}
\author[20]{B. Cimmino}
\author[13]{M. Clark}
\author[8]{A. P. Colijn}
\author[9]{J. Conrad}
\author[21]{J. J. Cuenca-Garc\'ia}
\author[16]{J. P. Cussonneau}
\author[22,14]{V. D'Andrea}
\author[8]{M. P. Decowski}
\author[3]{P. Di Gangi}
\author[8]{S. Di Pede}
\author[11]{A. Di Giovanni}
\author[20]{R. Di Stefano}
\author[16]{S. Diglio}
\author[15]{A. Elykov}
\author[23]{S. Farrell}
\author[22,14]{A. D. Ferella}
\author[15]{H. Fischer}
\author[7,14]{W. Fulgione}
\author[8]{P. Gaemers}
\author[4]{R. Gaior}
\author[12]{M. Galloway}
\author[24]{F. Gao}
\author[15]{R. Glade-Beucke}
\author[10]{L. Grandi}
\author[15]{J. Grigat}
\author[23]{A. Higuera}
\author[5]{C. Hils}
\author[19]{L. Hoetzsch}
\author[1]{J. Howlett}
\author[20]{M. Iacovacci}
\author[25]{Y. Itow}
\author[6]{J. Jakob}
\author[19]{F. Joerg}
\author[9]{A. Joy}
\author[2]{N. Kato}
\author[17]{P. Kavrigin}
\author[25]{S. Kazama\thanks{Also at Institute for Advanced Research, Nagoya University, Nagoya, Aichi 464-8601, Japan}}
\author[25]{M. Kobayashi}
\author[17]{G. Koltman}
\author[26]{A. Kopec}
\author[17]{H. Landsman}
\author[13]{R. F. Lang}
\author[17]{L. Levinson}
\author[23]{I. Li}
\author[13]{S. Li}
\author[23]{S. Liang}
\author[15]{S. Lindemann}
\author[19]{M. Lindner}
\author[24]{K. Liu}
\author[5]{F. Lombardi}
\author[10]{J. Long}
\author[18]{J. A. M. Lopes\thanks{Also at Coimbra Polytechnic - ISEC, 3030-199 Coimbra, Portugal}}
\author[26]{Y. Ma}
\author[22,14]{C. Macolino}
\author[9]{J. Mahlstedt}
\author[3]{A. Mancuso}
\author[11]{L. Manenti}
\author[12]{A. Manfredini}
\author[20]{F. Marignetti}
\author[19]{T. Marrod\'an Undagoitia}
\author[2]{K. Martens}
\author[16]{J. Masbou}
\author[15]{D. Masson}
\author[4]{E. Masson}
\author[20]{S. Mastroianni}
\author[14]{M. Messina}
\author[27]{K. Miuchi}
\author[27]{K. Mizukoshi}
\author[7]{A. Molinario}
\author[2]{S. Moriyama}
\author[1]{K. Mor\aa}
\author[17]{Y. Mosbacher}
\author[1]{M. Murra}
\author[15]{J. M\"uller}
\author[26]{K. Ni}
\author[5]{U. Oberlack}
\author[17]{B. Paetsch}
\author[19]{J. Palacio}
\author[12]{R. Peres}
\author[10]{J. Pienaar}
\author[16]{M. Pierre}
\author[19]{V. Pizzella}
\author[1]{G. Plante}
\author[26]{J. Qi}
\author[13]{J. Qin}
\author[12,15]{D. Ram\'irez Garc\'ia}
\author[21]{S. Reichard}
\author[15]{A. Rocchetti}
\author[19]{N. Rupp}
\author[23]{L. Sanchez}
\author[18]{J. M. F. dos Santos}
\author[3]{G. Sartorelli}
\author[19]{J. Schreiner}
\author[6]{D. Schulte}
\author[6]{P. Schulte}
\author[6]{H. Schulze Ei{\ss}ing}
\author[15]{M. Schumann}
\author[4]{L. Scotto Lavina}
\author[3]{M. Selvi}
\author[3]{F. Semeria}
\author[5]{P. Shagin}
\author[1]{S. Shi}
\author[26]{E. Shockley}
\author[18]{M. Silva}
\author[19]{H. Simgen}
\author[2]{A. Takeda}
\author[9]{P.-L. Tan}
\author[19]{A. Terliuk}
\author[16]{D. Thers}
\author[15]{F. Toschi}
\author[7]{G. Trinchero}
\author[23]{C. Tunnell}
\author[15]{F. T\"onnies}
\author[21]{K. Valerius}
\author[12]{G. Volta}
\author[26]{Y. Wei}
\author[6]{C. Weinheimer}
\author[17]{M. Weiss}
\author[5]{D. Wenz}
\author[12]{C. Wittweg}
\author[19]{T. Wolf}
\author[1]{Z. Xu}
\author[2]{M. Yamashita}
\author[26]{L. Yang}
\author[1]{J. Ye}
\author[10]{L. Yuan}
\author[3]{G. Zavattini\thanks{Also at INFN, Sez. di Ferrara and Dip. di Fisica e Scienze della Terra, Universit\`a di Ferrara, via G. Saragat 1, Edificio C, I-44122 Ferrara (FE), Italy}}
\author[1]{Y. Zhang}
\author[26]{M. Zhong}
\author[1]{T. Zhu}
\affil[1]{Physics Department, Columbia University, New York, NY 10027, USA}
\affil[2]{Kamioka Observatory, Institute for Cosmic Ray Research, and Kavli Institute for the Phy sics and Mathematics of the Universe (WPI), University of Tokyo, Higashi-Mozumi, Kamioka, Hida, Gifu 506-1205, Japan}
\affil[3]{Department of Physics and Astronomy, University of Bologna and INFN-Bologna, 40126 Bologna, Italy}
\affil[4]{LPNHE, Sorbonne Universit\'{e}, CNRS/IN2P3, 75005 Paris, France}
\affil[5]{Institut f\"ur Physik \& Exzellenzcluster PRISMA$^{+}$, Johannes Gutenberg-Universit\"at Mainz, 55099 Mainz, Germany}
\affil[6]{Institut f\"ur Kernphysik, Westf\"alische Wilhelms-Universit\"at M\"unster, 48149 M\"unster, Germany}
\affil[7]{INAF-Astrophysical Observatory of Torino, Department of Physics, University  of  Torino and  INFN-Torino,  10125  Torino,  Italy}
\affil[8]{Nikhef and the University of Amsterdam, Science Park, 1098XG Amsterdam, Netherlands}
\affil[9]{Oskar Klein Centre, Department of Physics, Stockholm University, AlbaNova, Stockholm SE-10691, Sweden}
\affil[10]{Department of Physics \& Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\affil[11]{New York University Abu Dhabi - Center for Astro, Particle and Planetary Physics, Abu Dhabi, United Arab Emirates}
\affil[12]{Physik-Institut, University of Z\"urich, 8057  Z\"urich, Switzerland}
\affil[13]{Department of Physics and Astronomy, Purdue University, West Lafayette, IN 47907, USA}
\affil[14]{INFN-Laboratori Nazionali del Gran Sasso and Gran Sasso Science Institute, 67100 L'Aquila, Italy}
\affil[15]{Physikalisches Institut, Universit\"at Freiburg, 79104 Freiburg, Germany}
\affil[16]{SUBATECH, IMT Atlantique, CNRS/IN2P3, Universit\'e de Nantes, Nantes 44307, France}
\affil[17]{Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot 7610001, Israel}
\affil[18]{LIBPhys, Department of Physics, University of Coimbra, 3004-516 Coimbra, Portugal}
\affil[19]{Max-Planck-Institut f\"ur Kernphysik, 69117 Heidelberg, Germany}
\affil[20]{Department of Physics ``Ettore Pancini'', University of Napoli and INFN-Napoli, 80126 Napoli, Italy}
\affil[21]{Institute for Astroparticle Physics, Karlsruhe Institute of Technology, 76021 Karlsruhe, Germany}
\affil[22]{Department of Physics and Chemistry, University of L'Aquila, 67100 L'Aquila, Italy}
\affil[23]{Department of Physics and Astronomy, Rice University, Houston, TX 77005, USA}
\affil[24]{Department of Physics \& Center for High Energy Physics, Tsinghua University, Beijing 100084, China}
\affil[25]{Kobayashi-Maskawa Institute for the Origin of Particles and the Universe, and Institute for Space-Earth Environmental Research, Nagoya University, Furo-cho, Chikusa-ku, Nagoya, Aichi 464-8602, Japan}
\affil[26]{Department of Physics, University of California San Diego, La Jolla, CA 92093, USA}
\affil[27]{Department of Physics, Kobe University, Kobe, Hyogo 657-8501, Japan}


%\collaborator{XENON Collaboration\email{xenon@lngs.infn.it}}

%\date{\today} 
%
%% CHANGE
%\begin{abstract}
%\end{abstract}
%
%% <--- SNIP 
%\maketitle
%
%\end{document}


